An Empirical Study of End-to-End Video-Language Transformers with Masked Visual Modeling

Masked visual modeling (MVM) has been recently proven effective for visual pre-training. While similar reconstructive objectives on video inputs (e.g., masked frame modeling) have been explored in video-language (VidL) pre-training, previous studies fail to find a truly effective MVM strategy that can largely benefit the downstream performance. In this work, we systematically examine the potential of MVM in the context of VidL learning. Specifically, we base our study on a fully end-to-end VIdeO-LanguagE Transformer (VIOLET), where the supervision from MVM training can be backpropagated to the video pixel space. In total, eight different reconstructive targets of MVM are explored, from low-level pixel values and oriented gradients to high-level depth maps, optical flow, discrete visual tokens, and latent visual features. We conduct comprehensive experiments and provide insights into the factors leading to effective MVM training, resulting in an enhanced model VIOLETv2. Empirically, we show VIOLETv2 pre-trained with MVM objective achieves notable improvements on 13 VidL benchmarks, ranging from video question answering, video captioning, to text-to-video retrieval.

==> def.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vdelta{{\bm{\delta}}}
\def\vphi{{\bm{\phi}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\newcommand{\alphav}{{\boldsymbol \alpha}}
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tabs/2d_feature_models.tex <==
\begin{table}[t]
\centering
    \tablestyle{5pt}{1.2} 
    \def \w{20pt} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l c|ccccc}
        \shline
        Image Feature & Train & TGIF-Frame & \multicolumn{4}{c}{DiDeMo-Retrieval} \\
        \cmidrule(lr){3-3}\cmidrule(lr){4-7}
         Model & Data & Acc. & R1 & R5 & R10 & AveR \\
        \hline
        ResNet-50~\cite{he2016resnet} & IN-1K & \\ 
        Swin-T~\cite{liu2021swin} & IN-1K & \\
        Swin-B & IN-1K &  \\
        \rowcolor{lightgray}
         Swin-B & IN-22K & \siftgif & \sifdro & \sifdrf & \sifdrt & \sifaver \\
         Swin-L & IN-22K & \\
        \shline
    \end{tabular}
    }
    \vspace{-2ex}
    \caption{\textbf{Does image classification accuracy of the model used to extract 2D Feature for MVM target correlate with downstream VidL performance?}. All
variants are pre-trained on WebVid~\cite{bain2021frozen} with VTM+MLM+MVM (2d feature) for 5 epochs, using RM as the masking strategy. The final pre-training setting is highlighted in \colorbox{lightgray}{gray}.}
    \label{table:mvm-webvid-ic}
\end{table}


==> tabs/masking_ratio_webvid.tex <==
\begin{table}[t]
\centering
    \tablestyle{5pt}{1.1} 
    \def \w{20pt} 
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{c| ccccc}
        \shline
        \multirow{2}{*}{Masking Ratio} & TGIF-Frame & \multicolumn{4}{c}{DiDeMo-Retrieval} \\
        \cmidrule(lr){2-2}\cmidrule(lr){3-6}
         & Acc. & R1 & R5 & R10 & AveR \\
        \hline
         15\% & \siftgif & \sifdro & \sifdrf & \sifdrt & \sifaver\\
         % 0.20 & 68.7 & \\
         % {'r@1': '35.55', 'r@5': '63.74', 'r@10': '74.77', 'median': '3'}
         \rowcolor{lightgray}
          30\%  &  68.8 & \textbf{36.2} & \textbf{64.0} & \textbf{74.5} & \textbf{58.2}\\
          % 0.40 & \\
          45\% & \textbf{68.9} & 35.6 & 61.9 & 74.4 & 57.3 \\
          % 0.50  & 68.9 & 36.6 & 64.0 & 74.1 & 58.2\\
          % {'r@1': '36.57', 'r@5': '64.04', 'r@10': '74.06', 'median': '3'}\\
          60\%  & 68.1 & 34.1 & 63.9 & 74.6 & 57.5\\
          % {'r@1': '34.12', 'r@5': '63.94', 'r@10': '74.57', 'median': '3'}
          % 0.70 & 68.3 & 
          % {'r@1': '35.75', 'r@5': '62.72', 'r@10': '73.85', 'median': '3'}
          75\%  & 68.3 & 35.4 & 62.4 & 74.2 & 57.3 \\
          % {'r@1': '35.44', 'r@5': '62.41', 'r@10': '74.16', 'median': '3'}
        \shline
    \end{tabular}
    % }
    \vspace{-2ex}
    \caption{Impact of \textbf{masking ratio for MVM}. All
variants are pre-trained on WebVid~\cite{bain2021frozen} with VTM+MLM+MVM (2d feature) for 5 epochs, using RM as the masking strategy. The final pre-training setting is highlighted in \colorbox{lightgray}{gray}.}
    \label{table:mvm-webvid-m_ratio}
\end{table}

==> tabs/rebuttal/clip.tex <==
\begin{table}[H]
\centering \tablestyle{2pt}{1.0} \scriptsize
    %\def \w{20pt}
    % \resizebox{\linewidth}{!}{
    \vspace{-3ex}
    \begin{tabular}{ll| cccc}
        \hline
        MVM & \multirow{2}{*}{Settings}  & TGIF-Frame & \multicolumn{3}{c}{DiDeMo-Retrieval} \\
        \cmidrule(lr){3-3}\cmidrule(lr){4-6}
        target & & Acc. & R1 & R5 & R10 \\
        \hline
        CLIP & \multirow{2}{*}{Default (Table 1)} & 67.7 & 29.8 & 57.8 & 68.5 \\
        Swin-B &  & 68.8 & 35.1 & 63.3 & 73.1 \\
        \hline
        \multirow{5}{*}{CLIP} & lr $\times$ 2 &70.5  & 32.9 & 61.6 & 73.5 \\
        % & lr / 2 (1e-5) & 67.0 & 26.1 & 54.8 & 67.8 \\
        & masking ratio = 0.3 (Table 5) & 68.0 & 31.8 & 59.6 & 71.3 \\
        & loss type = $l_2$ (Table 5, appendix) & 68.3 & 30.1 & 59.1 & 71.0 \\
        & linear MVM head (Table 6, appendix) & 68.2 & 30.5 & 58.3 & 69.2\\
        \hline
       \multirow{2}{*}{Swin-B} & lr $\times$ 2 & \textbf{70.6} & 33.3 & 63.7 & \textbf{75.2}\\
       & masking ratio = 0.3 (Table 5)  & 68.8 & \textbf{36.2} & \textbf{64.0} & 74.5 \\
        \hline
    \end{tabular}
    \vspace{-3ex}
    \label{table:mvm-webvid-init}
\end{table}

==> tabs/rebuttal/deit.tex <==
\begin{table}[H]
 \centering \tablestyle{4pt}{1.0} \scriptsize
    % \resizebox{\columnwidth}{!}{%
    \vspace{-3ex}
    \begin{tabular}{l cc|cccc}
        \hline
        Image Feat. & Train & IN-1K & TGIF-Frame & \multicolumn{3}{c}{DiDeMo-Retrieval} \\
        \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-7}
         Model & Data & ACC@1 & Acc. & R1 & R5 & R10  \\
        \hline
        ResNet-50 & IN-1K & 76.1 & 67.3 & 29.1 & 58.1 & 69.3 \\
        DeiT & IN-1K & 83.4 & 68.4 & 31.4 & 59.4 & 72.2 \\
        Swin-B & IN-1K & 83.5 & 68.3 & \textbf{34.9} & \textbf{63.4} & \textbf{73.9} \\
        %\hline
        %\rowcolor{lightgray} Swin-B & IN-22K & 85.2  & \textbf{\siftgif} & \textbf{\sifdro} & \sifdrf & \textbf{\sifdrt} \\
        \hline
    \end{tabular}
    \vspace{-3ex}
    % }
    % \caption{\textbf{Comparing Swin-B vs. another SIF model (DEiT)} All variants are pre-trained on WebVid with VTM+MLM+MVM (SIF) for 5 epochs, using RM with 15\% as the masking strategy. The final pre-training setting is highlighted in \colorbox{lightgray}{gray}. 
    %\caption{\small \linjie{DEIT, ls 0.02 69.2, ls 0.04 68.9, ls 1, 67.2, retrieval results from ls 0.02}}
    \label{table:mvm-sif-deit}
\end{table}


==> tabs/rebuttal/dense.tex <==
\begin{table}[H]
\centering \tablestyle{5pt}{1.0} \scriptsize
    \vspace{-3ex}
    % \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l |cccc}
        \hline
        MVM Target& TGIF-Frame & \multicolumn{3}{c}{DiDeMo-Retrieval} \\
        \cmidrule(lr){2-2} \cmidrule(lr){3-5} & Acc. & R1 & R5 & R10 \\
        \hline
        TVF & 68.0 & 32.8 & 60.5 & 73.0 \\
        % ep1.5: {'r@1': '30.13', 'r@5': '61.80', 'r@10': '72.83', 'median': '3'}
        % ep2: {'r@1': '32.18', 'r@5': '62.72', 'r@10': '73.65', 'median': '3'}
        TVF-dense & 68.4 & 34.3 & 60.8 & 72.4\\
        %ep1.5: {'r@1': '31.66', 'r@5': '62.21', 'r@10': '72.83', 'median': '3'}
        %ep2:  {'r@1': '34.32', 'r@5': '63.02', 'r@10': '73.03', 'median': '3'}
        % TVF-B & 67.5  & 25.8  & 55.0  & 68.0  \\
        \rowcolor{lightgray}
        SIF  & \textbf{\siftgif} & \textbf{\sifdro} & \textbf{\sifdrf} & \textbf{\sifdrt} \\
        \hline
    \end{tabular}
    \vspace{-3ex}
    % }
    % \caption{\textbf{TVF vs. TVF-dense.} All variants are pre-trained on WebVid with VTM+MLM+MVM for 5 epochs, using RM with 15\% as the masking strategy. The final pre-training setting is highlighted in \colorbox{lightgray}{gray}. 
    % }
    \label{table:mvm-tvf-dense}
\end{table}

==> tabs/rebuttal/init.tex <==
\begin{table}[H]
\centering \tablestyle{5pt}{1.0} \scriptsize
    %\def \w{20pt}
    % \resizebox{\linewidth}{!}{
    \vspace{-3ex}
    \begin{tabular}{lc| cccc}
        \hline
        \multirow{2}{*}{Weight Init.} & MVM & TGIF-Frame & \multicolumn{3}{c}{DiDeMo-Retrieval} \\
        \cmidrule(lr){3-3}\cmidrule(lr){4-6}
        & on VL & Acc. & R1 & R5 & R10  \\
        \hline
        Random & \ding{53} & 55.9 & 5.6 & 19.9 & 29.8 \\
        &  \checkmark &  56.5 & 7.4 & 22.9 & 33.8 \\
        %\hline
        %Swin~\cite{liu2021swin} &\ding{53} & 68.0 & 31.7 & 61.7 & 72.0 & 55.1\\
        %&  \checkmark & 68.0 & 31.7 & 60.7 & 70.7 %& 54.3\\
        \hline
        V-only MVM (TVF) & \ding{53} & 59.9 & 15.3 & 38.4 & 54.7 \\
        % {'r@1': '15.32', 'r@5': '38.41', 'r@10': '54.65', 'median': '9'}
        & \checkmark & 60.2  & 17.4 & 43.2  & 56.0 \\
        \hline
        V-only MVM (SIF) & \ding{53} & 61.0 & 16.9 & 42.4 & 54.9 \\
        & \checkmark & 61.5  & 18.6 & 44.0 & 58.1 \\
        %\hline
        %Swin~\cite{liu2021swin} &\ding{53} & 68.0 & 31.7 & 61.7 & 72.0 & 55.1\\
        %&  \checkmark & 68.0 & 31.7 & 60.7 & 70.7 %& 54.3\\
        \hline
        VidSwin-B &\ding{53} & 68.1 & 28.7 & 57.0 & 69.7 \\
        \rowcolor{lightgray} & \checkmark & \textbf{68.8} & \textbf{35.1} & \textbf{63.3} & \textbf{73.1} \\
        \hline
    \end{tabular}
    \vspace{-3ex}
    % }
%     \caption{Impact of \textbf{weight initialization of video backbone}. All
% variants are pre-trained on WebVid for 5 epochs. The MVM target for VidL pre-training is spatial-focused image features (SIF) from Swin-B, if not specified otherwise. The final pre-training setting is highlighted in \colorbox{lightgray}{gray}.}
    \label{table:mvm-webvid-init}
\end{table}


==> tabs/rebuttal/rebuttal_results.tex <==
% 3d/mvm_2d_clip_feature_mask0.3_lr4e-5_bsz36: 69.9 {'r@1': '34.73', 'r@5': '62.61', 'r@10': '73.03', 'median': '3'}
% 3d/mvm_2d_clip_feature_mask0.3_lr1e-5_bsz36: 67.0 {'r@1': '26.05', 'r@5': '54.75', 'r@10': '67.82', 'median': '5'}
% 3d/mvm_2d_clip_feature_mask0.3_lr2e-5_bsz36: 68.8 {'r@1': '31.77', 'r@5': '59.55', 'r@10': '71.30', 'median': '3'}
% 3d/mvm_2d_clip_feature_mvm_loss_l2_bsz36_a100: 68.3, {'r@1': '31.56', 'r@5': '60.47', 'r@10': '72.42', 'median': '3'}
% 3d/mvm_2d_clip_feature_bsz36_linear_head_a100: 69.4, {'r@1': '33.30', 'r@5': '62.61', 'r@10': '74.46', 'median': '3'}
% clip l2: {'r@1': '30.13', 'r@5': '59.14', 'r@10': '70.99', 'median': '4'}
% clip lr 4e-5: {'r@1': '32.89', 'r@5': '61.59', 'r@10': '73.54', 'median': '3'}
% clip linear head: {'r@1': '32.48', 'r@5': '61.49', 'r@10': '72.11', 'median': '3'}
% clip mask 0.3 ep_2_3: {'r@1': '28.60', 'r@5': '58.94', 'r@10': '71.71', 'median': '3'}
% clip mask 0.15 ep_2_3:  {'r@1': '29.52', 'r@5': '59.65', 'r@10': '71.09', 'median': '4'}
% clip 2e-5: {'r@1': '31.77', 'r@5': '61.08', 'r@10': '71.40', 'median': '3'}
% swin-b l2: 68.8 33.0 60.1 71.9 55.0
% swin-b linear head 68.8 31.3 60.1 72.8
% lr 4e-5: {'r@1': '33.30', 'r@5': '63.74', 'r@10': '75.18', 'median': '3'}
